Measurement of the forward-backward asymmetry in $Z/\gamma^{\ast} \rightarrow \mu^{+}\mu^{-}$ decays and determination of the effective weak mixing angle

The forward-backward charge asymmetry for the process $q\bar{q} \rightarrow Z/\gamma^{\ast} \rightarrow \mu^{+}\mu^{-}$ is measured as a function of the invariant mass of the dimuon system. Measurements are performed using proton proton collision data collected with the LHCb detector at $\sqrt{s} = 7$ and 8\tev, corresponding to integrated luminosities of $1$fb$^{-1}$ and $2$fb$^{-1}$ respectively. Within the Standard Model the results constrain the effective electroweak mixing angle to be $$sin^{2}\theta_{W}^{eff} = 0.23142 \pm 0.00073 \pm 0.00052 \pm 0.00056 $$ where the first uncertainty is statistical, the second systematic and the third theoretical. This result is in agreement with the current world average, and is one of the most precise determinations at hadron colliders to date.

==> LHCb_HD_comma_separated_author_2015-07-14.tex <==
LHCb collaboration:
R. Aaij, 
B. Adeva, 
M. Adinolfi, 
A. Affolder, 
Z. Ajaltouni, 
S. Akar, 
J. Albrecht, 
F. Alessio, 
M. Alexander, 
S. Ali, 
G. Alkhazov, 
P. Alvarez Cartelle, 
A.A. Alves Jr, 
S. Amato, 
S. Amerio, 
Y. Amhis, 
L. An, 
L. Anderlini, 
J. Anderson, 
G. Andreassi, 
M. Andreotti, 
J.E. Andrews, 
R.B. Appleby, 
O. Aquines Gutierrez, 
F. Archilli, 
P. d'Argent, 
A. Artamonov, 
M. Artuso, 
E. Aslanides, 
G. Auriemma, 
M. Baalouch, 
S. Bachmann, 
J.J. Back, 
A. Badalov, 
C. Baesso, 
W. Baldini, 
R.J. Barlow, 
C. Barschel, 
S. Barsuk, 
W. Barter, 
V. Batozskaya, 
V. Battista, 
A. Bay, 
L. Beaucourt, 
J. Beddow, 
F. Bedeschi, 
I. Bediaga, 
L.J. Bel, 
V. Bellee, 
N. Belloli, 
I. Belyaev, 
E. Ben-Haim, 
G. Bencivenni, 
S. Benson, 
J. Benton, 
A. Berezhnoy, 
R. Bernet, 
A. Bertolin, 
M.-O. Bettler, 
M. van Beuzekom, 
A. Bien, 
S. Bifani, 
P. Billoir, 
T. Bird, 
A. Birnkraut, 
A. Bizzeti, 
T. Blake, 
F. Blanc, 
J. Blouw, 
S. Blusk, 
V. Bocci, 
A. Bondar, 
N. Bondar, 
W. Bonivento, 
S. Borghi, 
M. Borsato, 
T.J.V. Bowcock, 
E. Bowen, 
C. Bozzi, 
S. Braun, 
M. Britsch, 
T. Britton, 
J. Brodzicka, 
N.H. Brook, 
E. Buchanan, 
A. Bursche, 
J. Buytaert, 
S. Cadeddu, 
R. Calabrese, 
M. Calvi, 
M. Calvo Gomez, 
P. Campana, 
D. Campora Perez, 
L. Capriotti, 
A. Carbone, 
G. Carboni, 
R. Cardinale, 
A. Cardini, 
P. Carniti, 
L. Carson, 
K. Carvalho Akiba, 
G. Casse, 
L. Cassina, 
L. Castillo Garcia, 
M. Cattaneo, 
Ch. Cauet, 
G. Cavallero, 
R. Cenci, 
M. Charles, 
Ph. Charpentier, 
M. Chefdeville, 
S. Chen, 
S.-F. Cheung, 
N. Chiapolini, 
M. Chrzaszcz, 
X. Cid Vidal, 
G. Ciezarek, 
P.E.L. Clarke, 
M. Clemencic, 
H.V. Cliff, 
J. Closier, 
V. Coco, 
J. Cogan, 
E. Cogneras, 
V. Cogoni, 
L. Cojocariu, 
G. Collazuol, 
P. Collins, 
A. Comerma-Montells, 
A. Contu, 
A. Cook, 
M. Coombes, 
S. Coquereau, 
G. Corti, 
M. Corvo, 
B. Couturier, 
G.A. Cowan, 
D.C. Craik, 
A. Crocombe, 
M. Cruz Torres, 
S. Cunliffe, 
R. Currie, 
C. D'Ambrosio, 
E. Dall'Occo, 
J. Dalseno, 
P.N.Y. David, 
A. Davis, 
O. De Aguiar Francisco, 
K. De Bruyn, 
S. De Capua, 
M. De Cian, 
J.M. De Miranda, 
L. De Paula, 
P. De Simone, 
C.-T. Dean, 
D. Decamp, 
M. Deckenhoff, 
L. Del Buono, 
N. D\'{e}l\'{e}age, 
M. Demmer, 
D. Derkach, 
O. Deschamps, 
F. Dettori, 
B. Dey, 
A. Di Canto, 
F. Di Ruscio, 
H. Dijkstra, 
S. Donleavy, 
F. Dordei, 
M. Dorigo, 
A. Dosil Su\'{a}rez, 
D. Dossett, 
A. Dovbnya, 
K. Dreimanis, 
L. Dufour, 
G. Dujany, 
F. Dupertuis, 
P. Durante, 
R. Dzhelyadin, 
A. Dziurda, 
A. Dzyuba, 
S. Easo, 
U. Egede, 
V. Egorychev, 
S. Eidelman, 
S. Eisenhardt, 
U. Eitschberger, 
R. Ekelhof, 
L. Eklund, 
I. El Rifai, 
Ch. Elsasser, 
S. Ely, 
S. Esen, 
H.M. Evans, 
T. Evans, 
A. Falabella, 
C. F\"{a}rber, 
N. Farley, 
S. Farry, 
R. Fay, 
D. Ferguson, 
V. Fernandez Albor, 
F. Ferrari, 
F. Ferreira Rodrigues, 
M. Ferro-Luzzi, 
S. Filippov, 
M. Fiore, 
M. Fiorini, 
M. Firlej, 
C. Fitzpatrick, 
T. Fiutowski, 
K. Fohl, 
P. Fol, 
M. Fontana, 
F. Fontanelli, 
R. Forty, 
M. Frank, 
C. Frei, 
M. Frosini, 
J. Fu, 
E. Furfaro, 
A. Gallas Torreira, 
D. Galli, 
S. Gallorini, 
S. Gambetta, 
M. Gandelman, 
P. Gandini, 
Y. Gao, 
J. Garc\'{i}a Pardi\~{n}as, 
J. Garra Tico, 
L. Garrido, 
D. Gascon, 
C. Gaspar, 
R. Gauld, 
L. Gavardi, 
G. Gazzoni, 
D. Gerick, 
E. Gersabeck, 
M. Gersabeck, 
T. Gershon, 
Ph. Ghez, 
S. Gian\`{i}, 
V. Gibson, 
O.G. Girard, 
L. Giubega, 
V.V. Gligorov, 
C. G\"{o}bel, 
D. Golubkov, 
A. Golutvin, 
A. Gomes, 
C. Gotti, 
M. Grabalosa G\'{a}ndara, 
R. Graciani Diaz, 
L.A. Granado Cardoso, 
E. Graug\'{e}s, 
E. Graverini, 
G. Graziani, 
A. Grecu, 
E. Greening, 
S. Gregson, 
P. Griffith, 
L. Grillo, 
O. Gr\"{u}nberg, 
B. Gui, 
E. Gushchin, 
Yu. Guz, 
T. Gys, 
T. Hadavizadeh, 
C. Hadjivasiliou, 
G. Haefeli, 
C. Haen, 
S.C. Haines, 
S. Hall, 
B. Hamilton, 
X. Han, 
S. Hansmann-Menzemer, 
N. Harnew, 
S.T. Harnew, 
J. Harrison, 
J. He, 
T. Head, 
V. Heijne, 
K. Hennessy, 
P. Henrard, 
L. Henry, 
E. van Herwijnen, 
M. He\ss, 
A. Hicheur, 
D. Hill, 
M. Hoballah, 
C. Hombach, 
W. Hulsbergen, 
T. Humair, 
N. Hussain, 
D. Hutchcroft, 
D. Hynds, 
M. Idzik, 
P. Ilten, 
R. Jacobsson, 
A. Jaeger, 
J. Jalocha, 
E. Jans, 
A. Jawahery, 
F. Jing, 
M. John, 
D. Johnson, 
C.R. Jones, 
C. Joram, 
B. Jost, 
N. Jurik, 
S. Kandybei, 
W. Kanso, 
M. Karacson, 
T.M. Karbach, 
S. Karodia, 
M. Kecke, 
M. Kelsey, 
I.R. Kenyon, 
M. Kenzie, 
T. Ketel, 
E. Khairullin, 
B. Khanji, 
C. Khurewathanakul, 
S. Klaver, 
K. Klimaszewski, 
O. Kochebina, 
M. Kolpin, 
I. Komarov, 
R.F. Koopman, 
P. Koppenburg, 
M. Kozeiha, 
L. Kravchuk, 
K. Kreplin, 
M. Kreps, 
G. Krocker, 
P. Krokovny, 
F. Kruse, 
W. Krzemien, 
W. Kucewicz, 
M. Kucharczyk, 
V. Kudryavtsev, 
A. K. Kuonen, 
K. Kurek, 
T. Kvaratskheliya, 
D. Lacarrere, 
G. Lafferty, 
A. Lai, 
D. Lambert, 
G. Lanfranchi, 
C. Langenbruch, 
B. Langhans, 
T. Latham, 
C. Lazzeroni, 
R. Le Gac, 
J. van Leerdam, 
J.-P. Lees, 
R. Lef\`{e}vre, 
A. Leflat, 
J. Lefran\c{c}ois, 
E. Lemos Cid, 
O. Leroy, 
T. Lesiak, 
B. Leverington, 
Y. Li, 
T. Likhomanenko, 
M. Liles, 
R. Lindner, 
C. Linn, 
F. Lionetto, 
B. Liu, 
X. Liu, 
D. Loh, 
I. Longstaff, 
J.H. Lopes, 
D. Lucchesi, 
M. Lucio Martinez, 
H. Luo, 
A. Lupato, 
E. Luppi, 
O. Lupton, 
A. Lusiani, 
F. Machefert, 
F. Maciuc, 
O. Maev, 
K. Maguire, 
S. Malde, 
A. Malinin, 
G. Manca, 
G. Mancinelli, 
P. Manning, 
A. Mapelli, 
J. Maratas, 
J.F. Marchand, 
U. Marconi, 
C. Marin Benito, 
P. Marino, 
J. Marks, 
G. Martellotti, 
M. Martin, 
M. Martinelli, 
D. Martinez Santos, 
F. Martinez Vidal, 
D. Martins Tostes, 
A. Massafferri, 
R. Matev, 
A. Mathad, 
Z. Mathe, 
C. Matteuzzi, 
A. Mauri, 
B. Maurin, 
A. Mazurov, 
M. McCann, 
J. McCarthy, 
A. McNab, 
R. McNulty, 
B. Meadows, 
F. Meier, 
M. Meissner, 
D. Melnychuk, 
M. Merk, 
E Michielin, 
D.A. Milanes, 
M.-N. Minard, 
D.S. Mitzel, 
J. Molina Rodriguez, 
I.A. Monroy, 
S. Monteil, 
M. Morandin, 
P. Morawski, 
A. Mord\`{a}, 
M.J. Morello, 
J. Moron, 
A.B. Morris, 
R. Mountain, 
F. Muheim, 
D. M\"{u}ller, 
J. M\"{u}ller, 
K. M\"{u}ller, 
V. M\"{u}ller, 
M. Mussini, 
B. Muster, 
P. Naik, 
T. Nakada, 
R. Nandakumar, 
A. Nandi, 
I. Nasteva, 
M. Needham, 
N. Neri, 
S. Neubert, 
N. Neufeld, 
M. Neuner, 
A.D. Nguyen, 
T.D. Nguyen, 
C. Nguyen-Mau, 
V. Niess, 
R. Niet, 
N. Nikitin, 
T. Nikodem, 
A. Novoselov, 
D.P. O'Hanlon, 
A. Oblakowska-Mucha, 
V. Obraztsov, 
S. Ogilvy, 
O. Okhrimenko, 
R. Oldeman, 
C.J.G. Onderwater, 
B. Osorio Rodrigues, 
J.M. Otalora Goicochea, 
A. Otto, 
P. Owen, 
A. Oyanguren, 
A. Palano, 
F. Palombo, 
M. Palutan, 
J. Panman, 
A. Papanestis, 
M. Pappagallo, 
L.L. Pappalardo, 
C. Pappenheimer, 
W. Parker, 
C. Parkes, 
G. Passaleva, 
G.D. Patel, 
M. Patel, 
C. Patrignani, 
A. Pearce, 
A. Pellegrino, 
G. Penso, 
M. Pepe Altarelli, 
S. Perazzini, 
P. Perret, 
L. Pescatore, 
K. Petridis, 
A. Petrolini, 
M. Petruzzo, 
E. Picatoste Olloqui, 
B. Pietrzyk, 
T. Pila\v{r}, 
D. Pinci, 
A. Pistone, 
A. Piucci, 
S. Playfer, 
M. Plo Casasus, 
T. Poikela, 
F. Polci, 
A. Poluektov, 
I. Polyakov, 
E. Polycarpo, 
A. Popov, 
D. Popov, 
B. Popovici, 
C. Potterat, 
E. Price, 
J.D. Price, 
J. Prisciandaro, 
A. Pritchard, 
C. Prouve, 
V. Pugatch, 
A. Puig Navarro, 
G. Punzi, 
W. Qian, 
R. Quagliani, 
B. Rachwal, 
J.H. Rademacker, 
M. Rama, 
M.S. Rangel, 
I. Raniuk, 
N. Rauschmayr, 
G. Raven, 
F. Redi, 
S. Reichert, 
M.M. Reid, 
A.C. dos Reis, 
S. Ricciardi, 
S. Richards, 
M. Rihl, 
K. Rinnert, 
V. Rives Molina, 
P. Robbe, 
A.B. Rodrigues, 
E. Rodrigues, 
J.A. Rodriguez Lopez, 
P. Rodriguez Perez, 
S. Roiser, 
V. Romanovsky, 
A. Romero Vidal, 
J. W. Ronayne, 
M. Rotondo, 
J. Rouvinet, 
T. Ruf, 
P. Ruiz Valls, 
J.J. Saborido Silva, 
N. Sagidova, 
P. Sail, 
B. Saitta, 
V. Salustino Guimaraes, 
C. Sanchez Mayordomo, 
B. Sanmartin Sedes, 
R. Santacesaria, 
C. Santamarina Rios, 
M. Santimaria, 
E. Santovetti, 
A. Sarti, 
C. Satriano, 
A. Satta, 
D.M. Saunders, 
D. Savrina, 
M. Schiller, 
H. Schindler, 
M. Schlupp, 
M. Schmelling, 
T. Schmelzer, 
B. Schmidt, 
O. Schneider, 
A. Schopper, 
M. Schubiger, 
M.-H. Schune, 
R. Schwemmer, 
B. Sciascia, 
A. Sciubba, 
A. Semennikov, 
N. Serra, 
J. Serrano, 
L. Sestini, 
P. Seyfert, 
M. Shapkin, 
I. Shapoval, 
Y. Shcheglov, 
T. Shears, 
L. Shekhtman, 
V. Shevchenko, 
A. Shires, 
B.G. Siddi, 
R. Silva Coutinho, 
L. Silva de Oliveira, 
G. Simi, 
M. Sirendi, 
N. Skidmore, 
T. Skwarnicki, 
E. Smith, 
E. Smith, 
I.T. Smith, 
J. Smith, 
M. Smith, 
H. Snoek, 
M.D. Sokoloff, 
F.J.P. Soler, 
F. Soomro, 
D. Souza, 
B. Souza De Paula, 
B. Spaan, 
P. Spradlin, 
S. Sridharan, 
F. Stagni, 
M. Stahl, 
S. Stahl, 
S. Stefkova, 
O. Steinkamp, 
O. Stenyakin, 
S. Stevenson, 
S. Stoica, 
S. Stone, 
B. Storaci, 
S. Stracka, 
M. Straticiuc, 
U. Straumann, 
L. Sun, 
W. Sutcliffe, 
K. Swientek, 
S. Swientek, 
V. Syropoulos, 
M. Szczekowski, 
T. Szumlak, 
S. T'Jampens, 
A. Tayduganov, 
T. Tekampe, 
M. Teklishyn, 
G. Tellarini, 
F. Teubert, 
C. Thomas, 
E. Thomas, 
J. van Tilburg, 
V. Tisserand, 
M. Tobin, 
J. Todd, 
S. Tolk, 
L. Tomassetti, 
D. Tonelli, 
S. Topp-Joergensen, 
N. Torr, 
E. Tournefier, 
S. Tourneur, 
K. Trabelsi, 
M.T. Tran, 
M. Tresch, 
A. Trisovic, 
A. Tsaregorodtsev, 
P. Tsopelas, 
N. Tuning, 
A. Ukleja, 
A. Ustyuzhanin, 
U. Uwer, 
C. Vacca, 
V. Vagnoni, 
G. Valenti, 
A. Vallier, 
R. Vazquez Gomez, 
P. Vazquez Regueiro, 
C. V\'{a}zquez Sierra, 
S. Vecchi, 
J.J. Velthuis, 
M. Veltri, 
G. Veneziano, 
M. Vesterinen, 
B. Viaud, 
D. Vieira, 
M. Vieites Diaz, 
X. Vilasis-Cardona, 
V. Volkov, 
A. Vollhardt, 
D. Volyanskyy, 
D. Voong, 
A. Vorobyev, 
V. Vorobyev, 
C. Vo\ss, 
J.A. de Vries, 
R. Waldi, 
C. Wallace, 
R. Wallace, 
J. Walsh, 
S. Wandernoth, 
J. Wang, 
D.R. Ward, 
N.K. Watson, 
D. Websdale, 
A. Weiden, 
M. Whitehead, 
G. Wilkinson, 
M. Wilkinson, 
M. Williams, 
M.P. Williams, 
M. Williams, 
T. Williams, 
F.F. Wilson, 
J. Wimberley, 
J. Wishahi, 
W. Wislicki, 
M. Witek, 
G. Wormser, 
S.A. Wotton, 
S. Wright, 
K. Wyllie, 
Y. Xie, 
Z. Xu, 
Z. Yang, 
J. Yu, 
X. Yuan, 
O. Yushchenko, 
M. Zangoli, 
M. Zavertyaev, 
L. Zhang, 
Y. Zhang, 
A. Zhelezov, 
A. Zhokhov, 
L. Zhong, 
S. Zucchelli

